Who's Your Judge? On the Detectability of LLM-Generated Judgments

Large Language Model (LLM)-based judgments leverage powerful LLMs to efficiently evaluate candidate content and provide judgment scores. However, the inherent biases and vulnerabilities of LLM-generated judgments raise concerns, underscoring the urgent need for distinguishing them in sensitive scenarios like academic peer reviewing. In this work, we propose and formalize the task of judgment detection and systematically investigate the detectability of LLM-generated judgments. Unlike LLM-generated text detection, judgment detection relies solely on judgment scores and candidates, reflecting real-world scenarios where textual feedback is often unavailable in the detection process. Our preliminary analysis shows that existing LLM-generated text detection methods perform poorly given their incapability to capture the interaction between judgment scores and candidate content -- an aspect crucial for effective judgment detection. Inspired by this, we introduce \textit{J-Detector}, a lightweight and transparent neural detector augmented with explicitly extracted linguistic and LLM-enhanced features to link LLM judges' biases with candidates' properties for accurate detection. Experiments across diverse datasets demonstrate the effectiveness of \textit{J-Detector} and show how its interpretability enables quantifying biases in LLM judges. Finally, we analyze key factors affecting the detectability of LLM-generated judgments and validate the practical utility of judgment detection in real-world scenarios.

==> prompt_antique.tex <==


\begin{tcolorbox}[breakable, title={ANTIQUE Prompt (3-Way Relevance Ranking)}, label=antique:rank3]
\small
\ttfamily
Given a prompt and three responses, follow the rubric to assess relevance and rank the responses.

\vspace{3mm}
\#\# Rubric (per-response relevance score in [1, 4]):\
\textbf{4}: Reasonable and convincing; on par with or better than a likely correct answer.\
\textbf{3}: Possibly an answer, but not sufficiently convincing; a better-quality answer likely exists.\
\textbf{2}: Not an acceptable answer; unreasonable or does not address the question, but still on-topic.\
\textbf{1}: Completely out of context or nonsensical.

\vspace{3mm}
\#\# Prompt: [QUERY]

\vspace{3mm}
\#\# Response 1: [RESPONSE\_1]

\vspace{3mm}
\#\# Response 2: [RESPONSE\_2]

\vspace{3mm}
\#\# Response 3: [RESPONSE\_3]

\vspace{3mm}
Please output a valid JSON object using the following schema:
{
\hspace{3mm}"Rationale": \textless explanation for your judgment and ranking\textgreater,\
\hspace{3mm}"Response1 Score": \textless 1--4\textgreater,\
\hspace{3mm}"Response2 Score": \textless 1--4\textgreater,\
\hspace{3mm}"Response3 Score": \textless 1--4\textgreater,\
\hspace{3mm}"Ranking": \textless list of indices indicating best$\rightarrow$worst, e.g., [0,1,2]\textgreater
}

\vspace{3mm}
Formatted the abovementioned schema and produce the judgment JSON now.
\end{tcolorbox}

==> prompt_helpsteer2.tex <==
\begin{tcolorbox}[breakable, title={HelpSteer2 Prompt (Pointwise, 5-Dimension Scoring)}, label=hs2:pointwise]
\small
\ttfamily
Given a prompt and a response, follow the rubric to make a judgment.

\vspace{3mm}
\#\# Rubric:

Judge the response on five aspects: \textbf{helpfulness}, \textbf{correctness}, \textbf{coherence}, \textbf{complexity}, and \textbf{verbosity}.\

Assign each aspect a scalar score in \textbf{[0, 4]}.

\vspace{3mm}
\#\# Prompt: [PROMPT]

\vspace{3mm}
\#\# Response: [RESPONSE]

\vspace{3mm}
Please output a valid JSON object using the following schema:
{
\hspace{3mm}"Rationale": \textless explanation for the given scores\textgreater,\
\hspace{3mm}"Helpfulness": \textless 0--4\textgreater,\
\hspace{3mm}"Correctness": \textless 0--4\textgreater,\
\hspace{3mm}"Coherence": \textless 0--4\textgreater,\
\hspace{3mm}"Complexity": \textless 0--4\textgreater,\
\hspace{3mm}"Verbosity": \textless 0--4\textgreater
}

\vspace{3mm}
Formatted the abovementioned schema and produce the judgment JSON now.
\end{tcolorbox}

==> prompt_helpsteer3.tex <==



\begin{tcolorbox}[breakable, title={HelpSteer3 Prompt (Pairwise Comparison)}, label=hs3:pairwise]
\small
\ttfamily
Given a prompt and two responses, follow the rubric to make a comparative judgment.

\vspace{3mm}
\#\# Rubric:
Compare \textbf{Response 1} and \textbf{Response 2} along five aspects: \textbf{helpfulness}, \textbf{correctness}, \textbf{coherence}, \textbf{complexity}, and \textbf{verbosity}.\
Assign a single comparative score in {-3,-2,-1,0,1,2,3} using the scale: \
-3: R1 \textit{much better} than R2; \ \ -2: R1 \textit{better} than R2; \ \ -1: R1 \textit{slightly better} than R2; \
\phantom{-3:}\ 0: about the same; \ \ 1: R2 \textit{slightly better} than R1; \ \ 2: R2 \textit{better} than R1; \ \ 3: R2 \textit{much better} than R1.

\vspace{3mm}
\#\# Prompt (conversation/context):\
[CONTEXT AS FLATTENED TEXT]

\vspace{3mm}
\#\# Response 1:\
[RESPONSE\_1]

\vspace{3mm}
\#\# Response 2:\
[RESPONSE\_2]

\vspace{3mm}
Please output a valid JSON object using the following schema:
{
\hspace{3mm}"Rationale": \textless explanation for the comparative score\textgreater,\
\hspace{3mm}"Score": \textless -3\textbar -2\textbar -1\textbar 0\textbar 1\textbar 2\textbar 3\textgreater
}

\vspace{3mm}
Formatted the abovementioned schema and produce the judgment JSON now.
\end{tcolorbox}

==> prompt_neurips.tex <==
\begin{tcolorbox}[breakable, title={NeurIPS Review Prompt (Structured JSON Review)}, label=neurips:review]
\small
\ttfamily
You are an AI researcher reviewing a paper submitted to a prestigious AI conference. Thoroughly evaluate the paper, adhering to the provided guidelines, and return a detailed assessment in the specified JSON format.

\vspace{3mm}
\#\# Manuscript: [MANUSCRIPT TEXT OR CONCATENATED CHUNKS]

\vspace{3mm}
\#\# Reviewer Guidelines (dimensions to cover):

\textbf{Summary}: Briefly summarize contributions (no critique here).\

\textbf{Strengths \& Weaknesses} across: Originality, Quality, Clarity, Significance.\

Provide \textbf{Questions} for authors (useful for rebuttal).\

Discuss \textbf{Limitations} and potential societal impact.\

Flag \textbf{Ethical Concerns} if applicable (per conference policy).\

Assign numerical ratings: \textbf{Soundness}, \textbf{Presentation}, \textbf{Contribution} (1--4 each).\

Provide an \textbf{Overall} score (1--10) and \textbf{Confidence} (1--5).

\vspace{3mm}
\#\# Output a valid JSON object with the following fields:
{
\hspace{3mm}"Summary": \textless summary for the paper\textgreater,\
\hspace{3mm}"Questions": \textless questions for the author\textgreater,\
\hspace{3mm}"Limitations": \textless limitations for the paper\textgreater,\
\hspace{3mm}"Soundness": \textless 1--4\textgreater,\
\hspace{3mm}"Presentation": \textless 1--4\textgreater,\
\hspace{3mm}"Contribution": \textless 1--4\textgreater,\
\hspace{3mm}"Overall": \textless 1--10\textgreater,\
\hspace{3mm}"Confidence": \textless 1--5\textgreater
}

\vspace{3mm}
Formatted the abovementioned schema and produce the review JSON now.
\end{tcolorbox}
